Automata Terms in a Lazy WSkS Decision Procedure (Technical Report)

We propose a lazy decision procedure for the logic WSkS. It builds a term-based symbolic representation of the state space of the tree automaton (TA) constructed by the classical WSkS decision procedure. The classical decision procedure transforms the symbolic representation into a TA via a bottom-up traversal and then tests its language non-emptiness, which corresponds to satisfiability of the formula. On the other hand, we start evaluating the representation from the top, construct the state space on the fly, and utilize opportunities to prune away parts of the state space irrelevant to the language emptiness test. In order to do so, we needed to extend the notion of language terms (denoting language derivatives) used in our previous procedure for the linear fragment of the logic (the so-called WS1S) into automata terms. We implemented our decision procedure and identified classes of formulae on which our prototype implementation is significantly faster than the classical procedure implemented in the Mona tool.

==> macros.tex <==

% theorems and lemmas
% \declaretheorem[name=Lemma,sharenumber=theorem]{mlemma}
% \declaretheorem[name=Theorem,sharenumber=mlemma]{mtheorem}


\makeatletter
\def\moverlay{\mathpalette\mov@rlay}
\def\mov@rlay#1#2{\leavevmode\vtop{%
   \baselineskip\z@skip \lineskiplimit-\maxdimen
   \ialign{\hfil$\m@th#1##$\hfil\cr#2\crcr}}}
\newcommand{\charfusion}[3][\mathord]{
    #1{\ifx#1\mathop\vphantom{#2}\fi
        \mathpalette\mov@rlay{#2\cr#3}
      }
    \ifx#1\mathop\expandafter\displaylimits\fi}
\makeatother

% Lukas's amazing transition symbol START
\makeatletter
\DeclareRobustCommand{\shorttox}{%
  \mathrel{\mathpalette\shortx@to\relax}%
}

\DeclareRobustCommand{\shortminusx}{%
  \mathrel{\mathpalette\shortx@minus\relax}%
}

\newcommand{\shortx@to}[2]{%
  \mkern2mu
  \clipbox{{.5\width} 0 0 0}{$\m@th#1\vphantom{+}{\rightarrow}$}%
}

\newcommand{\shortx@minus}[2]{%
  \mkern2mu
  \clipbox{{.5\width} 0 0 0}{$\m@th#1\vphantom{+}{-}$}%
}
\makeatother

\newcommand{\labeledto}[1]{{{\shortminusx}\hspace{-2pt}\raisebox{0.16ex}{$\scriptstyle\{ #1\hspace{-0.28pt}\}$}\hspace{-2.2pt}{\shorttox}}}
\newcommand{\scriptlabeledto}[1]{{{\shortminusx}\hspace{-1.0pt}\raisebox{0.12ex}{$\scriptscriptstyle\{ #1\hspace{-0.28pt}\}$}\hspace{-1.6pt}{\shorttox}}}
\newcommand\ltrxx[1]{%standard LaTex syntax where each parameter is put in {}
\mathchoice
{\,\labeledto{#1}\,}
{\labeledto{#1}}
{\scriptlabeledto{#1}}
{\scriptlabeledto{#1}}
}
% Lukas's amazing transition symbol END

\newcommand{\sct}[1]{\S{\ref{#1}}}

\newcommand{\cupdot}{\charfusion[\mathbin]{\cup}{\cdot}}
\newcommand{\capdot}{\charfusion[\mathbin]{\cap}{\cdot}}
% \newcommand{\hminus}[1]{\,\overline{\scriptstyle #1}\,}
% \newcommand{\hminus}[1]{\mathop{\stackrel[\raisebox{0mm}{$\scriptstyle #1$}]{}{-}}}
\newcommand{\hminus}[1]{\mathop{\ooalign{$-$\cr\raise-2pt\hbox{$\scriptstyle{} #1\mkern4mu$}\cr}}}

\newcommand{\vh}[1]{\textcolor{orange}{\ifmmode \text{[VH: #1]}\else [VH: #1] \fi}}
\newcommand{\ol}[1]{\textcolor{blue}{\ifmmode \text{[OL: #1]}\else [OL: #1] \fi}}
\newcommand{\lh}[1]{\textcolor{green}{\ifmmode \text{[LH: #1]}\else [LH: #1] \fi}}
\newcommand{\tv}[1]{\textcolor{magenta}{\ifmmode \text{[TV: #1]}\else [TV: #1] \fi}}

%\renewcommand{\vh}[1]{}
%\renewcommand{\ol}[1]{}
%\renewcommand{\lh}[1]{}
%\renewcommand{\tv}[1]{}

\newcommand{\secref}[1]{Section~\ref{#1}}

\newcommand{\nat}[0]{\mathbb{N}}
\newcommand{\wsks}{WS$k$S\xspace}
\newcommand{\pre}{\mathit{pre}}
\newcommand{\cpre}{\mathit{cpre}}
\newcommand{\post}{\mathit{post}}
\newcommand{\nxt}{\mathit{next}}
\newcommand{\fold}{\mathit{fold}}
\newcommand{\pad}{\mathit{pad}}
\newcommand{\prepad}{\mathit{prepad}}
\newcommand{\cprepad}{\mathit{cprepad}}
\newcommand{\arity}{\mathit{Arity}}
\newcommand{\fc}{\mathcal{F}}
\newcommand{\rc}{\mathcal{R}}
\newcommand{\pc}{\mathcal{P}}
\newcommand{\scl}{\mathcal{S}}

\newcommand{\dom}[0]{\mathrm{dom}}
\newcommand{\domof}[1]{\dom(#1)}
\newcommand{\img}[0]{\mathrm{img}}
\newcommand{\imgof}[1]{\img(#1)}
\newcommand{\pos}[0]{\mathrm{pos}}
\newcommand{\posof}[1]{\pos(#1)}

% left and right successors
\newcommand{\tleft}[0]{\mathtt{L}}
\newcommand{\tright}[0]{\mathtt{R}}
\newcommand{\leftright}[0]{\{\tleft, \tright\}}

% transitions
\newcommand{\ltr}[1]{\ltrxx{#1}} % labelled->

\newcommand{\varsof}[1]{\mathit{Vars}(#1)}   % variables of a formula


% chinese mu (木)character
\newcommand{\chinmu}{%
\tikzset{external/export next=false}
  \tikz[
    scale=0.9,
    transform shape
  ]{
    \path[use as bounding box] (-1.0mm,0mm) rectangle (1.0mm,2.0mm);
    %\draw (0mm,0mm) -- (0mm,5mm);
    \draw (0mm,0.1mm) -- (0mm,2.1mm);
    \draw (-1mm,1.5mm) -- (1mm,1.5mm);
    \draw (0mm,1.5mm) edge[bend left=15 ] (-0.9mm,0.4mm);
    \draw (0mm,1.5mm) edge[bend right=15] ( 0.9mm,0.4mm);
  }%
}

%now as a savebox
\newsavebox\chinmubox
\setbox0=\hbox{%
\tikzset{external/export next=false}
%\hspace*{-3.8mm}
\hspace*{-2.7mm}
\chinmu
%\Wintertree
%\Autumntree
%\Summertree
%\Springtree
}
\sbox\chinmubox{\copy0}

\newcommand{\simpletree}{{\rotatebox[origin=c]{90}{\text{\rm\guillemotright}}}}
%\renewcommand{\simpletree}{{\rotatebox[origin=c]{90}{\text{\guillemotright}\hspace{-2mm}-}}}
%\renewcommand{\simpletree}{{\rotatebox[origin=c]{90}{\text{\guillemotright}\hspace{-1.5mm}-\hspace{-1.7mm}-}}}
%\renewcommand{\simpletree}
%  {\reflectbox{\rotatebox[origin=c]{90}{\clipbox{{.5\width} 0 0 0}{$\twoheadrightarrow$}}}}

% all trees木
\newcommand{\alltrees}[0]{\alltreesx{\Sigma}}
\newcommand{\allzerotrees}[0]{\alltreesx{\zerosymb}}
% \newcommand{\allzerotrees}[0]{\alltreesx{\{\zerosymb\}}}
\newcommand{\allzerotreesx}[0]{\alltreesx{\{\zerosymbx\}}}
%\newcommand{\alltreesx}[1]{#1^{\chinmu}}
\newcommand{\alltreesx}[1]{#1^{\usebox\chinmubox}}
% \newcommand{\alltreesx}[1]{#1^{\usebox\chinmubox}}
%\newcommand{\alltreesx}[1]{#1^{\anothersimpletree}}
%\newcommand{\alltreesx}[1]{#1^{木}}
% \newcommand{\alltreesx}[1]{#1^{\simpletree}}
% \newcommand{\alltreesof}[1]{\alltreesx{\left\{#1\right\}}}
\newcommand{\alltreesof}[1]{\alltreesx{\{#1\}}}
% languages
% \newcommand{\lang}[0]{L}
\newcommand{\lang}[0]{\mathcal{L}}
\newcommand{\langp}[0]{\lang'}
% variables
\newcommand{\vars}[0]{\mathbb{X}}
\newcommand{\varsY}[0]{\mathbb{Y}}

\newcommand{\restr}[2]{#1_{|#2}}
\newcommand{\frestr}[1]{\restr{f}{#1}}

\newcommand{\spruce}%
  {\begin{tikzpicture}
     [every node/.style=
       {circle,draw,fill,minimum size=1.5pt,inner sep=0pt,outer sep=0pt},
      line cap=round
     ]
   \draw (0,0) -- (0,0.25) -- (0.1,0.15);
   \draw (0,0.25) -- (-0.1,0.15);
   \draw (0,0.15) -- (-0.1,0.05);
   \draw (0,0.15) -- (0.1,0.05);
   \end{tikzpicture}
  }

\newcommand{\gcl}{cl_\gamma}
\newcommand{\fh}{\zeta}
\newcommand{\stree}[1]{\spruce[#1]}

\newcommand{\tree}[0]{\tau}
\newcommand{\treeof}[1]{\tree_{#1}}
\newcommand{\treebot}[0]{\tree_{\bot}}


% \newcommand{\cyl}[0]{\Gamma}
\newcommand{\cyl}[0]{\mathcal{C}}
\newcommand{\cylof}[2]{\cyl_{#1}(#2)}
\newcommand{\complof}[1]{\overline{#1}}
\newcommand{\freeof}[1]{\mathit{free}(#1)}


\newcommand{\strans}[1]{\Delta_{#1}^\sharp}
\newcommand{\trans}[0]{\delta}
% \newcommand{\transof}[1]{\trans_{#1}}
\newcommand{\transof}[3]{\trans_{#3}(#1, #2)}
\newcommand{\Trans}[0]{\Delta}
\newcommand{\Transof}[3]{\Trans_{#3}(#1, #2)}
\newcommand{\zero}{\bar{0}}
\newcommand{\lf}[1]{L_{#1}}
\newcommand{\lfsharp}[1]{L_{#1}^\sharp}
\newcommand{\fin}[1]{F_{#1}}
\newcommand{\finsharp}[1]{F_{#1}^\sharp}
\newcommand{\nfin}[1]{N_{#1}}
\newcommand{\nfinsharp}[1]{N_{#1}^\sharp}

\newcommand{\dcset}[1]{\mathord\downarrow\{#1 \}}
\newcommand{\upkriglset}[1]{\mathord\uparrow{\textstyle\coprod\{#1\}}}
\newcommand{\kriglset}[1]{\textstyle\coprod\{#1\}}
\newcommand{\dcbb}[1]{\mathord\downarrow\mathbb{#1}}
\newcommand{\dccal}[1]{\mathord\downarrow\mathcal{#1}}
\newcommand{\upkriglbb}[1]{\mathord\uparrow\textstyle\coprod\mathbb{#1}}
\newcommand{\upkriglcal}[1]{{\mathord\uparrow\textstyle\coprod\mathcal{#1}}}
\newcommand{\bby}{\mathbb{Y}}

\newcommand{\aphi}[1]{A_{\varphi_{#1}}}
\newcommand{\aphisharp}[1]{A_{\varphi_{#1}^\sharp}}
\newcommand{\xvar}{\mathcal{X}}

\newcommand{\bs}{\mathit{bs}}
\newcommand{\cbs}{\mathit{cbs}}

\newcommand{\tablechoice}[8]{\begin{tabular}{|l|l|l|l|}
\hline
 #1 & #2 & #3 & #4  \\ \hline
 #5 & #6 & #7 & #8 \\ \hline
\end{tabular}}

\newcommand{\limplies}[0]{\mathrel{\Rightarrow}}
\newcommand{\linvimplies}[0]{\mathrel{\Leftarrow}}
\newcommand{\liff}[0]{\mathrel{\iff}}
% a call tree to be used on a line
\newcommand{\treeonelay}[3]{\tikz[anchor=base,baseline,sibling distance=6mm,%
  level distance=4mm,inner sep=0.4mm,yshift=2mm,%
%  every node/.style={circle,draw}%
  ]{%
    \scriptsize%
    \node {$#1$} child {node {$#2$}} child {node {$#3$}}}%
  }

\newcommand{\up}{\mathsf{up}}
\newcommand{\dotsym}[1]{#1^{\bullet}}
\newcommand{\crosssym}[1]{#1^{\times}}
\newcommand{\botsym}[1]{#1^{\bot}}
\newcommand{\captimes}{\charfusion[\mathbin]{\cap}{\scriptscriptstyle\times}}
\newcommand{\minterm}{\mathcal M}
\newcommand{\determ}{\mathsf{det}}
\newcommand{\canon}{\mathsf{can}}

\newcommand{\aut}{\mathsf{aut}}
\newcommand{\term}[0]{t}

%%%%%%%%%%% hojja hojaaaaaaa
%\newcommand{\termof}[1]{\term_{#1}}
%\newcommand{\autof}[1]{\A_{#1}}
%\newcommand{\translof}[1]{\langle#1\rangle}
%\newcommand{\langof}[1]{\lang(#1)}
%\newcommand{\seman}[1]{\left\llbracket #1 \right\rrbracket}
%
\newcommand{\termof}[1]{t_{#1}}
\newcommand{\autof}[1]{\A_{#1}}
\newcommand{\translof}[1]{\langle #1\rangle}
\newcommand{\langof}[1]{\lang\left(#1\right)}
\newcommand{\langpof}[1]{\langp\left(#1\right)}
\newcommand{\langofreasonable}[1]{\lang(#1)}
\newcommand{\seman}[1]{\langof{#1}}
\newcommand{\semanreasonable}[1]{\langofreasonable{#1}}




\newcommand{\conj}{\mathop{\text{\scriptsize\&}}}
\newcommand{\disj}{\mathop{+}}
%\newcommand{\seman}[1]{\langof{#1}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\Q}{\mathcal{Q}}
% USED?
% \newcommand{\Lf}{\mathcal{L}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\cX}{\mathcal{X}}

\def\underbrak#1{\mathop{\vtop{\ialign{##\crcr
$\hfil\displaystyle{#1}\hfil$\crcr\noalign{\kern3\p@\nointerlineskip}
\upbracketfill\crcr\noalign{\kern3\p@}}}}\limits}

% \newcommand{\timesof}[1]{\mathop{\times_{[#1]}}}
% \newcommand{\timesof}[1]{\mathop{\times}\limits^{\scriptscriptstyle[#1]}}
\newcommand{\timesof}[1]{\mathop{[#1]}}
%\newcommand{\timesof}[1]{\times_{#1}}
% \newcommand{\timesof}[1]{\mathop{\times_{(#1)}}}
\newcommand{\atom}[0]{\mathit{atom}}
%\newcommand{\translof}[1]{t_{#1}}
%\newcommand{\translof}[1]{q(#1)}
\newcommand{\leafsof}[1]{\mathit{Leaf}(#1)}

%\newcommand{\rt}[0]{\mathit{root}}
\newcommand{\rt}[0]{\mathcal{R}}
\newcommand{\rtof}[1]{\rt(#1)}
\newcommand{\expand}[1]{\mathit{expand}(#1)}

\newcommand{\msquare}{\mathord{\scalebox{0.7}{\scalerel*{\Box}{gX}}}}

\newcommand{\leafs}[0]{I}
\newcommand{\roots}[0]{R}
\newcommand{\sing}{\mathrm{Sing}}
\newcommand{\singof}[1]{\sing(#1)}
% successor
\newcommand{\suck}[0]{S}
\newcommand{\suckof}[2]{\suck_{#1}(#2)}
\newcommand{\suckleftof}[1]{\suckof{\tleft}{#1}}
\newcommand{\suckrightof}[1]{\suckof{\tright}{#1}}
\newcommand{\suckleftrightof}[1]{\suckof{\tleft/\tright}{#1}}

% symbols
\newcommand{\symb}[0]{\xi}
\newcommand{\unitrack}[2]{\left[\!\begin{array}{rl} \scriptstyle #1:&\scriptstyle #2\end{array}\!\right]}
\newcommand{\bintrack}[4]{\left[\resizebox{!}{3.5mm}{$\begin{array}{rl} #1:&#3\\ #2:&#4\end{array}$}\right]}
\newcommand{\bintracknolab}[2]{{\resizebox{!}{3.5mm}{\ensuremath{\begin{array}{l} #1\\#2\end{array}}}}}


% alphabet
\newcommand{\alphof}[1]{\Sigma_{#1}}
\newcommand{\zerosymb}[0]{\overline{0}}
\newcommand{\zerosymbvars}[1]{\overline{0}_{#1}}
\newcommand{\zerosymbx}[0]{\zerosymbvars{\vars}}

% \renewcommand{\zerosymb}[0]{\bar{0}}
% \renewcommand{\zerosymbvars}[1]{\bar{0}_{#1}}

\renewcommand{\zerosymb}[0]{\vec{0}}
\renewcommand{\zerosymbvars}[1]{\vec{0}_{#1}}


% shared TikZ definitions
\tikzstyle{varnode}=[emptynode,rectangle split, rounded corners, rectangle split parts=2,
  rectangle split horizontal,rectangle split part align=base,inner sep=0.8mm, draw, align=center,fill=none]
\tikzstyle{emptynode}=[draw,circle,fill=black,inner sep=0.2mm]
\tikzstyle{bluenode}=[emptynode,inner sep=0.8mm,draw=blue,fill=blue!50]
\tikzstyle{voidnode}=[emptynode,draw=none,fill=none]
\tikzstyle{varnodeno}=[varnode,rectangle split part fill={black!15,black!15}]
\newcommand{\parted}[2]{#1\nodepart{two}#2}

\newcommand{\context}{\mathbb{C}}
\newcommand{\contextx}{\mathbb{C}[X]}
\newcommand{\bbt}{\mathbb{T}}
\newcommand{\calt}{\mathcal{T}}

\newcommand{\saturof}[1]{#1^{\mathsf{s}}}
% \newcommand{\saturof}[1]{S^{[#1]}}
\newcommand{\expt}[1]{#1^{\mathsf{e}}}
\newcommand{\emptysymb}[0]{\overline{0}}
\newcommand{\emp}{\mathit{emp}}

%\newcommand\ssucc[2]{\cup_{q\in #1,r\in #1}\Delta_#2(q,r)}
\newcommand\ssucc[2]{\Delta_#2(#1)}
\newcommand{\fixpoint}[2]{\mu Z. #1 \cup \ssucc{Z}{\beta}}
\newcommand{\fixpointset}[2]{\mu Z. #1 \cup Z\ominus #2 }

\newcommand{\append}[0]{\cdot}
\newcommand{\appendP}[0]{\cdot_{P}}
\newcommand{\leav}{\mathit{leaf}}

% reachable states
\newcommand{\reach}[0]{\mathit{reach}}
\newcommand{\reachof}[2]{\reach_{#2}(#1)}
\newcommand{\reachxof}[3]{\reach_{#2}(#1, #3)}


% experimental evaluation
%\newcommand{\tomo}[0]{\textsc{To/Mo}}
\newcommand{\tomo}[0]{--}
\newcommand{\edge}[0]{\mathit{edge}}
\newcommand{\edgeL}[0]{\mathit{edge}_{\tleft}}
\newcommand{\edgeR}[0]{\mathit{edge}_{\tright}}
\newcommand{\edgeLR}[0]{\mathit{edge}_{\tleft/\tright}}

% \newcommand{\syms}[0]{\Theta}
\newcommand{\syms}[0]{\Gamma}          % set of symbols (used in quotient)
\newcommand{\allterms}[0]{\calt}       % set of all terms

\newcommand{\defeq}[0]{\mathrel{\stackrel{\text{def}}{=}}}  % defining =
\newcommand{\defequiv}[0]{\mathrel{\stackrel{\text{def}}{\Leftrightarrow}}} % defining equivalence

\newcommand{\subst}[2]{[#1/#2]} % substitution

% tools
\newcommand{\mona}[0]{\textsc{Mona}\xspace}
\newcommand{\osel}[0]{\textsc{jMosel}\xspace}
\newcommand{\gaston}[0]{\textsc{Gaston}\xspace}
\newcommand{\libvata}[0]{\textsc{Vata}\xspace}
\newcommand{\dwina}[0]{\textsc{dWiNA}\xspace}
\newcommand{\toss}[0]{\textsc{Toss}\xspace}
\newcommand{\traytel}[0]{\textsc{Coalg}\xspace}
\newcommand{\veanes}[0]{\textsc{SFA}\xspace}
%

\newcommand\typeof[1]{\mathsf{tp}(#1)}
\newcommand\type{\mathsf{tp}}
\newcommand{\tpclassof}[1]{[#1]_\type}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% a short mapsto
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\DeclareRobustCommand{\shortto}{%
  \mathrel{\mathpalette\short@to\relax}%
}

\DeclareRobustCommand{\shortfrom}{%
  \mathrel{\mathpalette\short@from\relax}%
}

\newcommand{\short@to}[2]{%
  \mkern2mu
  \clipbox{{.6\width} 0 0 0}{$\m@th#1\vphantom{+}{\mapsto}$}%
}

\newcommand{\short@from}[2]{%
  \mkern2mu
  \clipbox{0 0 {.8\width} 0  }{$\m@th#1\vphantom{+}{\mapsto}$}%
}
\makeatother

\newcommand{\shortmapsto}{{\shortfrom}\hspace{-0.5mm}{\shortto}}

\renewcommand{\unitrack}[2]{ \{ { #1\!\shortmapsto #2} \}}
\renewcommand{\bintrack}[4]{\biggl\{\!\begin{array}{r@{\!\shortmapsto}l} #1&#3,\\[-1.2mm] #2&#4\end{array}\!\biggr\}}
%\renewcommand{\bintrack}[4]{\begin{array}{r@{\!\shortmapsto}l} \{#1&#3,\\[-1.2mm] #2&#4\}\end{array}}
%\renewcommand{\bintrack}[4]{\resizebox{!}{3.5mm}{$\begin{array}{rl} #1\shortmapsto&#3\\ #2\shortmapsto&#4\end{array}$}}


%\newcommand{\asgn}[0]{\eta}    % assignment to variables
\newcommand{\asgn}[0]{\nu}    % assignment to variables
\newcommand{\proj}[0]{\pi}     % projection
\newcommand{\projof}[2]{\proj_{#1}(#2)}     % projection of ... over ...
\newcommand{\pump}[0]{\kappa}    % pumping of symbols with new tracks
\newcommand{\pumpof}[2]{\pump_{#1}(#2)} % pumping of symbols with new tracks

\newcommand{\minenc}[0]{\treeof \asgn ^{\mathit{min}}}  % minimum encoding

\newcommand{\rwr}[0]{\mathrel{\leadsto}}   % rewrites to
\newcommand{\subsum}[0]{\mathrel{\sqsubseteq}}   % subsumption
\newcommand{\subsumfe}[0]{\mathrel{\subsum^{\forall\exists}}}   % subsumption for all exists
% \newcommand{\subsetof}[1]{#1^{\subseteq}}   % rewrites to
\newcommand{\subsetof}[1]{#1^{\mathcal{D}}}   % rewrites to

\newcommand{\true}[0]{\mathit{true}}  % true
\newcommand{\false}[0]{\mathit{false}}  % false

\newcommand{\interf}[0]{\mathrel{\bowtie}}  % the interference operator

\newcommand{\theiof}[1]{\mathit{d}(#1)}

\newcommand{\pspace}[0]{\mathsf{PSPACE}\xspace}    % PSPACE
\newcommand{\exptime}[0]{\mathsf{EXPTIME}\xspace}    % EXP

\newcommand{\aterm}[0]{A}
\newcommand{\sterm}[0]{S}

